Conic locus of inversive Poncelet circumcenter and two points of invariant circle power

We prove that over a generic Poncelet triangle family, the locus of the circumcenter of an inversive triangle is a conic. Additionally, we prove an earlier conjecture: over generic Poncelet triangles, two unique points exist which maintain constant power with respect to the circumcircle and Euler's circle of the family, respectively.

==> 000_setup.tex <==
\usepackage{mathptmx}
%\setmainfont{TeX Gyre Termes}
%\setmathfont{TeX Gyre Termes Math}
\usepackage[margin=1.25in]{geometry}
\linespread{0.95}
\makeatletter
% Redefine \section to reduce spacing
%\def\section{\@startsection{section}{1}%
%  \z@{1.5ex \@plus 0.5ex \@minus 0.5ex}%
%  {1ex \@plus 0.2ex}%
%  {\normalfont\bfseries}}
%\makeatother

\usepackage{graphics}
\usepackage{thmtools}
\usepackage{wasysym}
%\usepackage{arxiv}
%\usepackage{enseign}
%\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage{amsthm}
\usepackage{amsbsy,amsmath,amssymb,amscd,amsfonts}
\usepackage{xstring}
\usepackage{hyperref}
%\usepackage[nameinlink,capitalize,noabbrev]{cleveref}

\DeclareRobustCommand{\hrefs}[1]{%
  \def\temphrefsurl{#1}% Store the full URL
  \IfBeginWith{\temphrefsurl}{http://}{%
    \StrGobbleLeft{\temphrefsurl}{7}[\temphrefsdisplayurl]% Remove "http://" (7 chars)
  }{%
    \IfBeginWith{\temphrefsurl}{https://}{%
      \StrGobbleLeft{\temphrefsurl}{8}[\temphrefsdisplayurl]% Remove "https://" (8 chars)
    }{%
      % Fallback if neither http:// nor https:// is found
      \def\temphrefsdisplayurl{\temphrefsurl}% Display the full URL as is
    }%
  }%
  \href{\temphrefsurl}{\texttt{\temphrefsdisplayurl}}% Create the link
}

\usepackage{graphicx,float,latexsym,color}
\usepackage[export]{adjustbox}

%\usepackage{mathspec}
\usepackage[font={scriptsize,it},skip=5pt]{caption}
\newcommand{\zcaption}[1]{
\captionsetup{width=0.9\linewidth}\caption{#1}}
\usepackage{subcaption}
%\let\proof\relax
%\let\endproof\relax

\usepackage{makecell}
\renewcommand{\arraystretch}{1.2}

\usepackage[dvipsnames]{xcolor}

\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{observation}{Observation}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{question}{Question}
\hypersetup{
%    pagebackref=false,
    %bookmarks=true,         % show bookmarks bar?
    %unicode=true,          % non-Latin characters in Acrobat’s bookmarks
    pdftoolbar=true,        % show Acrobat’s toolbar?
    pdfmenubar=true,        % show Acrobat’s menu?
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of 
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=OliveGreen,          % color of internal links (change box color with linkbordercolor)
    citecolor=blue,        % color of links to bibliography
    filecolor=black,      % color of file links
    urlcolor=red           % color of external links
}

\usepackage{listings}
\usepackage{lineno}
\def\linenumberfont{\normalfont\small\sffamily}
%a4: 210 x 297
%\textwidth=125mm
%\textheight=195mm
\arraycolsep=2pt
\captionsetup{width=120mm}

\newcommand{\tc}[2]{\textcolor{#1}{#2}}
\newcommand{\tb}[1]{\textbf{#1}}
%\newcommand{\tr}[1]{\tc{Red}{to do}}
\newcommand{\tr}[1]{\tc{Red}{#1}}
\newcommand{\ti}[1]{\textit{#1}}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}
 
\usepackage{comment}
\usepackage{microtype}
\usepackage{footnote}
%\usepackage{tablefootnote}
%\usepackage{longtable}

%\usepackage{night}

\renewcommand{\O}{\mathcal{O}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\F}{\mathcal{F}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\Q}{\mathcal{Q}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\D}{\mathbb{D}}
\renewcommand{\T}{\mathcal{T}}
\newcommand{\Tt}{\T_{\triangle}}
\newcommand{\To}{\T_{\circ}}
\newcommand{\Et}{\E_{\triangle}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\Rm}{\mathcal{R}}
\newcommand{\Cp}{\mathbb{C}}
\newcommand{\ol}{\overline}
\renewcommand{\l}{\lambda}
\newcommand{\X}{\mathcal{X}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\gP}{P^{\dagger}}
\newcommand{\gL}{\L^{\dagger}}

\newcommand{\torp}[2]{\texorpdfstring{#1}{#2}}
\newcommand{\ab}{_{\alpha,\beta}}
\newcommand{\rc}{\raisebox{0.3ex}{,}}
\newcommand{\rd}{\raisebox{0.3ex}{.}}

\usepackage{breqn}
\setlength{\mathindent}{0pt}
\renewcommand{\eqnumfont}{\normalfont}

\newcommand{\tightmath}[1]{%
  \begingroup
    \thinmuskip=0mu
    \medmuskip=0mu
    \thickmuskip=0mu
    #1%
  \endgroup
}
\setlength{\fboxsep}{0pt}  % Padding inside the frame

\newcommand{\twofigs}[4]{%
  \begin{figure}[htbp]
    \centering
    \fbox{%
      \begin{minipage}[c]{0.98\textwidth}
        \centering
        \hfill
        \begin{minipage}[c]{0.45\textwidth}
          \centering
          \vspace{5pt}
          \includegraphics[width=\linewidth]{#1}
          \vspace{0pt}
        \end{minipage}%
        \hspace{0.5em}
        \vrule width 0.5pt
        \hspace{0.5em}
        \begin{minipage}[c]{0.45\textwidth}
          \centering
          \vspace{5pt}
          \includegraphics[width=\linewidth]{#2}
          \vspace{0pt}
        \end{minipage}
        \hfill
      \end{minipage}
    }
    \caption{#3}
    \label{#4}
  \end{figure}
}

% does not work with cleveref
%\renewcommand{\cref}[1]{\ref{#1}}
%\usepackage{refcheck}

% alternative to refcheck, works with cleveref
%\usepackage[outer]{showlabels}
%\renewcommand{\showlabelfont}{\small\color{red}\ttfamily}


